STanHop: Sparse Tandem Hopfield Model for Memory-Enhanced Time Series Prediction

We present STanHop-Net (Sparse Tandem Hopfield Network) for multivariate time series prediction with memory-enhanced capabilities. At the heart of our approach is STanHop, a novel Hopfield-based neural network block, which sparsely learns and stores both temporal and cross-series representations in a data-dependent fashion. In essence, STanHop sequentially learn temporal representation and cross-series representation using two tandem sparse Hopfield layers. In addition, StanHop incorporates two additional external memory modules: a Plug-and-Play module and a Tune-and-Play module for train-less and task-aware memory-enhancements, respectively. They allow StanHop-Net to swiftly respond to certain sudden events. Methodologically, we construct the StanHop-Net by stacking STanHop blocks in a hierarchical fashion, enabling multi-resolution feature extraction with resolution-specific sparsity. Theoretically, we introduce a sparse extension of the modern Hopfield model (Generalized Sparse Modern Hopfield Model) and show that it endows a tighter memory retrieval error compared to the dense counterpart without sacrificing memory capacity. Empirically, we validate the efficacy of our framework on both synthetic and real-world settings.

==> 2theory.tex <==
In this section, we generalize the Gini entropic regularizer in sparsemax-based Hopfield model, i.e. $\Psi(\bp)\coloneqq \half \sum_\mu^M p_\mu(1-p_\mu)$, as Tsallis $\alpha$-entropies
\bea
\Psi^\alpha(\bp)\coloneqq
\begin{cases}
\frac{1}{\alpha(\alpha-1)}\sum_\mu^M (\bp_\mu-\bp_\mu^\alpha), \text{ for } \alpha>1\\
-\sum_{\mu}^M\bp_\mu\log\bp_\mu, \text{ for } \alpha=1
\end{cases}
\eea
proposed in \cite{tsallis1988possible}, where $\alpha$ represents the sparsity of probability distribution.
Based on the convex conjugate of the generalized entropic regularizer, we propose a generalized sparse Hopfield energy and sparse retrieval dynamics to analyze the sparsity-induced properties in the modern Hopfield model.

\subsection{Convergence of Generalized Sparse Hopfield Energy}

In order to discuss the sparsity-dependent properties, we inherit the Hopfield energy function from our previous work:
\bea
\label{eqn:H_entmax}
\calH(\bx)=-\Psi^\star\(\beta \bm{\bm{\Xi}}^\sT \bx\) +\half \Braket{\bx,\bx},
\eea
where $\Psi^\star(\cdot)$ denotes convex conjugate of entropic regularizer and $\alpha$-entmax is defined for $\bz \in \R^M$.
\begin{definition}[Variational form of $\alpha$-entmax \cite{peters2019sparse}]
\bea
\alphaentmax \coloneqq \argmax_{\bp \in \Delta^M} [\bp^\sT z+\Psi^{\alpha}(\bp)],
\eea
where $\Psi^{\alpha}(\bp)=\frac{1}{\alpha(\alpha-1)}\sum^M_{\mu=1}p_\mu-p_\mu^\alpha$ is the Tsallis entropic regularizer.
\end{definition}
\begin{definition}[Closed-form of $\alpha$-entmax]
For $\bz \in \R^M$, the $\alpha$-entmax transformation can be defined as
\bea
\alphaentmax=[(\alpha-1)\bz-\tau(\bz)]^{\frac{1}{\alpha-1}},
\eea
where we denote $[t]_{+}\coloneqq \max\{t,0\}$, and $\tau$ is the unique function $\R^M \to \R$ such that $\sum^M_{\mu=1}[(\alpha-1)\bz-\tau(\bz)]^{\frac{1}{\alpha-1}}$ satisfies the probability distribution.
\end{definition}
Since the computation of $\alpha$-entmax in closed form relies on the choice of $\alpha$, we will discuss these special cases, i.e. 1-entmax (Softmax), 1.5-entmax and 2-entmax (Sparsemax), to analyze the impact of sparsity on modern Hopfield model.
\begin{definition}
\label{def:convex_conjugate}
Suppose $F(\bp,\bz)\coloneqq\Braket{\bp,\bz}-\Psi^\alpha(\bp)$. Then the convex conjugate of $\Psi^\alpha$, $\Psi^\star$ takes the form:
\bea
\Psi^\star(\bz)=\Max_{\bp\in\Delta^M}\Braket{\bp,\bz}-\Psi^\alpha(\bp)=\Max_{\bp\in\Delta^M}F(\bp,\bz),
\eea
with $\Psi^\alpha$ being the Tsallis entropic regularizer.
\end{definition}
\begin{lemma}[Convex Conjugate of Entropic Regularizer]
\label{lemma:convex conjugate}
Given the convex conjugate of $\Psi^\alpha$ defined in \cref{def:convex_conjugate}. Then, the function $\Psi^\star$ is convex and its partial derivative can be formulated as:
\bea
\grad \Psi^\star(\bz)=\alphaentmax(\bz),
\eea
that is, the $\alphaentmax$ of the input vector $\bz$.
\end{lemma}
\cref{lemma:convex conjugate} not only provide the intuition behind the sparse Hopfield energy \eqref{eqn:H_entmax} --- the memory patterns are stored in local minima aligned with the overlap-function constructions (i.e.  $\norm{\bm{\bm{\Xi}}^\sT \bx}^2=\sumM \Braket{\bxi_\mu, \bx}^2$) in \cite{ramsauer2020hopfield,demircigil2017model,krotov2016dense} --- but also inspire us for the following corresponding generalized retrieval dynamics.
\begin{proof}
By Danskin's theorem \cite{danskin2012theory, bertsekas1999nonlinear}, the function $\Psi^\star$ is convex and its partial derivative with respect to $\bz$ is equal to that of $F$, i.e.$\nicefrac{\partial \Psi^\star}{\partial \bz}=\nicefrac{\partial F}{\partial \bz}$, if the following three conditions are satisfied for $\Psi^\star$ and $F$.
\begin{enumerate}
    \item [(i)]
    $F(\bp,\bz):\bP\times \R^M$ is a continuous function, where $\bP\subset\R^M$ is a compact set.
    \item [(ii)]
    The function $F$ is convex in $\bz$, i.e. for each given $\bp\subset\bP$, the mapping $\bz\to F(\bp,\bz)$ is convex.
    \item [(iii)]
    There exists an unique maximizing point $\hat{\bp}$ such that $F(\hat{\bp},\bz)=\Max_{\bp\in\bP}F(\bp,\bz)$.
\end{enumerate}

Since both $\Braket{\bp,\bz}$ and $\Psi^\alpha$ are continuous functions and every component of $\bp$ is ranging from $0$ to $1$, i.e. $\bp_\mu\in[0,1]$ for all $\mu\in M$, the function $F$ is continuous and the domain $\bP$ is a compact set.
Therefore, condition (i) is satisfied. 
For given probability distribution $\bp$, $F(\bp,\bz)=\Braket{\bp,\bz}-\Psi^\alpha(\bp)$ reduces to an affine function depending on input $\bz$.
Since affine function is convex, condition (ii) holds for all given $\bp\subset\bP$. 
Since for a given $\bz$, $\alphaentmax$ only produces an unique corresponding probability distribution $\bp^\star$, condition (iii) must be satisfied. 
Therefore, from Danskin's theorem, the function $\Psi^\star$ is convex and differentiable, and derivative of $\Psi^\star$ can be formulated as:
\bea
\grad_z \Psi^\star(\bz)=\frac{\partial F}{\partial \bz}=\frac{\partial}{\partial \bz}(\Braket{\bp,\bz}-\Psi^\alpha(\bp))=\bp=\alphaentmax(\bz).
\eea
\end{proof}
\begin{lemma}[Generalized retrieval dynamics]
Let $t$ denote the iteration step. The retrieval dynamics
\bea
\label{eqn:entmax_retrieval_dyn}
\bx_{t+1}
=
\calT\(\bx_t\)
\coloneqq
\grad_\bx\Psi\(\beta\bm{\bm{\Xi}}^\sT \bx\)\big\vert_{\bx_{t}}
=
\bm{\bm{\Xi}} \alphaentmax\(\beta\bm{\bm{\Xi}}^\sT \bx_t\)
\eea
can lead the energy function $\calH$ to decrease with respect to the increasing $t$, i.e. $\calH(\bx_{t+1})\leq\calH(\bx_t)$.
\end{lemma}


\begin{definition} [Stored and Retrieved]
\label{def:stored_and_retrieved}
Assuming that every pattern $\bxi_\mu$ surrounded by a sphere $S_\mu$ with finite radius $R\coloneqq \half \Min_{\mu,\nu\in[M]}\norm{\bxi_\mu-\bxi_\nu}$, we say $\bxi_\mu$ is \textit{stored} if there exists a generalized fixed point of $\calT$, $\bx^\star_\mu \in S_\mu$, to which all limit points $\bx \in S_\mu$ converge to, and $S_\mu \cap S_\nu=\emptyset$ for $\mu \neq \nu$. 
We say $\bxi_\mu$ is $\epsilon$-\textit{retrieved} by $\calT$ with $\bx$ for an error\footnote{The retrieval error has a naive bound $\epsilon\coloneqq\Max\big\{\norm{\bx-\bxi_\mu},\norm{\bxi_\mu-\bx^\star_\mu}\big\}$ by interpolating from $\bx$ to $\bxi_\mu$.} $\epsilon$, if $\norm{\calT(\bx)-\bxi_\mu}\le \epsilon$.
\end{definition}
\begin{lemma}[Convergence of Retrieval Dynamics $\calT$]
\label{lemma:convergence_sparse}
Given the energy function$\calH$ and retrieval dynamics $\calT(\bx)$ defined in \eqref{eqn:H_entmax} and \eqref{eqn:entmax_retrieval_dyn}, respectively.
For any sequence $\{\mathbf{x}_t\}_{t=0}^{\infty}$ generated by the iteration $\mathbf{x}_{t'+1} = \mathcal{T}(\mathbf{x}_{t'})$, all limit points of this sequence are stationary points of $\calH$.
\end{lemma}
To prove the convergence property of retrieval dynamics $\calT$, first we introduce two auxiliary lemmas from \cite{gunawardana2005convergence} and \cite{sriperumbudur2009convergence}.
\begin{lemma}[\cite{gunawardana2005convergence}, Proposition 7]
    \label{Second condition of generalizaed fixed points}
    Let $\calH_U: \calX_{t} \times \calX_{t+1}$ and $\calT: \calX_t \to \calX_{t+1}$ be a real-valued continuous function and a point-to-set mapping, respectively. We define
    \begin{align}
    \calT(\bx_{t}) &\coloneqq \argmin_{\bx'_{t+1} \in \calX_{t+1}} \calH_U(\bx_t,\bx'_{t+1})\\
    &= \{\bx_{t+1} \;\vert\; \calH_U(\bx_t,\bx_{t+1}) \leq \calH_U(\bx_t,\bx'_{t+1}), \forall \bx'_{t+1}\in \calX_{t+1} \},
    \end{align}
    where $\bx_t\in\calX_t$ and $\bx_{t+1}\in\calX_{t+1}$.
    Then, if $\calT(\bx)$ is non-empty, the mapping $\calT$ is a closed at $\bx_t$ .
    \end{lemma}
\begin{lemma}[\cite{sriperumbudur2009convergence}, Lemma 5]
\label{KKT for stationary points}
Following \cref{lemma:convergence_sparse}, $\bx$ is called the fixed point of iteration $\calT$ with respect to $\calH$ if $\bx = \calT(\bx)$ and is considered as a generalized fixed point of $\calT$ if $\bx\in\calT(\bx)$.
If $\bx^\star$ is a generalized fixed point of $\calT$, then, $\bx^\star$ is a stationary point of the energy minimization problem  \eqref{eqn:energy_minimizaiton}.
\end{lemma}

\begin{proof}
 On the basis of Zangwill global convergence theory for iterative algorithms \cite{zangwill1969nonlinear}, all limit points of $\{\bx_t\}^\infty_{t=0}$ are fixed points\footnote{Recall that, a fixed point of $\calT$ is defined as $\bx^\star \coloneqq \{\bx\;|\; \bx=\calT(\bx^\star)\}$.}, if the following three conditions are satisfied for the energy function $\calH$ and the retrieval dynamics $\calT$.
    \begin{enumerate}
        \item [(i)] 
        For any sequence $\{\mathbf{x}_t\}_{t=0}^{\infty}$ with starting point $\bx_0\in S_\mu$, 
        all points are in the same compact set $S_\mu$.
        \item [(ii)] $\calH$ is monotonically decreased by $\calT(\bx)$, i.e. $\calH(\bx_{t+1}) \leq \calH(\bx_t), \forall \bx_{t+1}=\calT(\bx_t)$.
        \item [(iii)] For all $t$, if $\calH(\bx_{t+1})<\calH(\bx_t)$, $\calT$ is closed at $\bx_t$.
    \end{enumerate}
    
    Furthermore, $\lim_{t \to \infty} \calH\(\bx_t\)=\calH\(\bx^\star\)$ for all limit points $\bx^\star$.

    By \cref{def:stored_and_retrieved}, 
    since $S_\mu$ with finite radius $R$ is bounded and closed, every $S_\mu$ is a compact set.
    Namely, for any sequence $\{\mathbf{x}_t\}_{t=0}^{\infty}$, all points are embedded in the sphere $S_\mu$, which is a compact set. Therefore, condition (i) is automatically satisfied. Then condition (ii), the monotonic descent property of $\{\bx_t\}^\infty_{t=0}$, has been analyzed in the original paper of CCCP \cite{yuille2003concave}. 
    By our definition on $\calH_1$ and $\calH_2$, we have $\calH_U\(\bx,\by\) \coloneqq \calH_1(\bx)+\calH_2(\by)  +\Braket{(\bx-\by),\grad_\bx \calH_2(\by)}$ is continuous in $\bx$ and $\by$. Consequently, by Lemma \ref{Second condition of generalizaed fixed points}, the non-empty assumption of the point-to-set map $\calT$ guarantees that $\calT$ is closed at $\bx_t$ and so satisfies condition (iii) for generalized fixed points. Therefore, by Zangwill global convergence theory, all the limit points of $\{\bx_t\}^\infty_{t=0}$ are generalized fixed points and $\lim_{t \to \infty} \calH\(\bx_t\)=\calH\(\bx^\star\)$, where $\bx^\star$ are some generalized fixed points of $\calT$. Furthermore, based on the results of Lemma \ref{KKT for stationary points}, $x^\star$ are also the stationary points of the minimization problem \eqref{eqn:energy_minimizaiton}. Therefore, the energy function is ensured to converge to local optimum.
\end{proof}

\begin{definition}[Separation of Patterns]
\label{def:separation_of_patterns}
The separation of a memory pattern $\bxi_\mu$ from all other memory patterns $\bm{\Xi}$ is defined as its minimal inner product difference to any other patterns:
\vspace{3pt}
\bea
\label{eqn:sep_delta_mu}
\Delta_\mu\coloneqq
\Min_{\nu,\nu\neq \mu}\[\Braket{\bxi_\mu,\bxi_\mu}-\Braket{\bxi_\mu,\bxi_\nu}\]=\Braket{\bxi_\mu,\bxi_\mu}-\Max_{\nu,\nu\neq \mu }\[\Braket{\bxi_\mu,\bxi_\nu}\].
\eea
Similarly, the separation of $\bxi_\mu$ at a given $\bx$ from all memory patterns $\bm{\Xi}$ is given by
\bea
\label{eqn:tilde_sep_delta_mu}
\Tilde{\Delta}_\mu\coloneqq
\Min_{\nu,\nu\neq \mu}\[\Braket{\bx,\bxi_\mu}-\Braket{\bx,\bxi_\nu}\].
\eea    
\end{definition}
\begin{theorem}[Retrieval Error]
\label{coro:eps_sparse_dense}
Let $\calT_{\text{Dense}}$ be the retrieval dynamics of the dense modern Hopfield model \cite{ramsauer2020hopfield}.
It holds
\begin{align}
\label{eqn:eps_sparse_dense}
\norm{\calT(\bx)-\bxi_\mu} 
\leq
\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}
\leq  2m(M-1) \exp{-\beta \(\Braket{\bxi_\mu,\bx}-\Max_{\nu\in[M]}\Braket{\bxi_\mu,\bxi_\nu}\)}.
\end{align}
for all $\bx\in S_\mu$.
\end{theorem}

\begin{proof}
We observe
\begin{align}
&\norm{\calT(\bx)-\bxi_\mu}-\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}\nonumber\\
&=\norm{\sum_{\nu=1}^{\kappa} \bxi_\nu \[\text{$(\alpha+\delta)$-entmax}\(\beta \bm{\Xi}^\sT \bx\) \]_\nu-\bxi_\mu}
-\norm{\sum_{\nu=1}^{\kappa} \bxi_\nu \[\alphaentmax\(\beta \bm{\Xi}^\sT \bx\) \]_\nu-\bxi_\mu}\\
&\leq
\norm{\sum^{\kappa}_{\nu=1}\[\text{$(\alpha+\delta)$-entmax}(\beta\bm{\Xi}^\sT \bx)\]_\nu\bxi_\nu }-
\norm{\sum^{\kappa}_{\nu=1} \[\alphaentmax\(\beta \bm{\Xi}^\sT \bx\)\]_\nu \bxi_\nu}\leq 0,
\end{align}
which gives
\bea
\label{eqn:eps_sparse_dense}
\norm{\calT(\bx)-\bxi_\mu} 
&\leq& 
\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}.
\eea
Then, we formulate the upper bound on $\norm{\calT_{\text{dense}}(\bx)-\bxi_\mu}$:
\begin{align}
\norm{\calT_{\text{dense}}(\bx)-\bxi_\mu}
&=
\norm{\sum_{\nu=1}^M [\Softmax(\beta\bm{\Xi}^\sT\bx)]_\nu\bxi_\nu-\bxi_\mu}\\
&=
\norm{\sum_{\nu=1, \nu\neq\mu}^M[\Softmax(\beta\bm{\Xi}^\sT\bx)]_\nu\bxi_\nu-(1-\Softmax(\beta\bm{\Xi}^\sT\bx))\bxi_\mu}\\
&\leq
\frac{\Tilde{\epsilon}}{M-1}\sum_{\nu=1, \nu\neq\mu}^M\norm{\bxi_\nu}+\Tilde{\epsilon}\norm{\bxi_\mu}\\
&\leq
\frac{\Tilde{\epsilon}(M-1)}{M-1}m+\Tilde{\epsilon}m\\
&=
2\Tilde{\epsilon}m,
\end{align}
where $\tilde{\epsilon}\coloneqq (M-1)\exp{-\beta \tilde{\Delta}_\mu}
=(M-1)\exp{-\beta \(\Braket{\bxi_\mu,\bx}-\Max_{\nu\in[M]}\Braket{\bxi_\mu,\bxi_\nu}\)}
$ and the upper bound on Softmax function
\bea
\[\Softmax(\beta \Xi^\sT \bx)\]_\nu
=\frac{\exp{\beta\(\Braket{\bx,\bxi_\nu}-\Braket{\bx,\bxi_\mu}\)}}{1+\sum_{\nu'\neq \mu} \exp{\beta\(\Braket{\bx,\bxi_{\nu'}}-\Braket{\bx,\bxi_\mu}\)}}
\le 
\exp{-\beta \Tilde{\Delta}_\mu},
\eea 
is used in the fourth line.
\end{proof}

Intuitively, the larger sparsity leads the lower retrieval error.
\begin{corollary}
\label{coro:error_1}
Let $\calT_{\text{Dense}}$ be the retrieval dynamics of the dense modern Hopfield model \cite{ramsauer2020hopfield}.
Suppose $\calT$ is given by \cref{lemma:retrieval_dyn} and its $\alpha\in (1,2)$. 
Then the retrieval error has an upper bound
\bea
\norm{\calT(\bx)-\bxi_\mu}\leq2m(M-1) \exp{-\beta \(\Braket{\bxi_\mu,\bx}-\Max_{\nu\in[M]}\Braket{\bxi_\mu,\bxi_\nu}\)}.
\eea
\end{corollary}
\begin{proof}
Recall the first inequality of \cref{coro:eps_sparse_dense}, which states that
\bea
\norm{\calT(\bx)-\bxi_\mu}\leq\norm{\calT_{dense}(\bx)-\bxi_\mu}.
\eea
\end{proof}
\begin{corollary}
\label{coro:eps_sparse_over_2}
Suppose $\alpha\geq 2$ and the retrieval dynamics is given by \cref{lemma:retrieval_dyn}. Then the retrieval error takes the upper bound:
\bea
\label{eqn:eps_sparse_over_2}
\norm{\calT(\bx)-\bxi_\mu}\leq m+d^{\nicefrac{1}{2}}m\beta \[\kappa \(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}\)+\frac{1}{\beta}\]
\eea
\end{corollary}
\begin{proof}
Following the setting of $\alphaentmax$ in \cite{peters2019sparse}, the equation
\bea
2-\text{entmax}(\beta\bm{\Xi}^\sT\bx)=\Sparsemax(\beta\bm{\Xi}^\sT\bx)
\eea
holds.
According to the closed form solution of $\Sparsemax$ in \cite{martins2016softmax}, 
it holds
\begin{align}
[ \Sparsemax \(\beta \bm{\Xi}^\sT \bx\) ]_\mu 
&\le 
\[\beta \bm{\Xi}^\sT \bx \]_{\mu}-\[\beta \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\kappa},
\label{eqn:sparsemax_upper_identity}
\end{align}
for all $\mu\in[M]$.
Then, the sparsemax retrieval error is 
\begin{align}
\norm{\calT_{\Sparsemax}\(\bx\)-\bxi^\mu}&=
\norm{\bm{\bm{\Xi}}\Sparsemax\(\beta \bm{\bm{\Xi}}^\sT \bx\)-\bxi^\mu}
=\norm{\sum_{\nu=1}^{\kappa} \bxi_{(\nu)} \[\Sparsemax\(\beta \bm{\bm{\Xi}}^\sT \bx\) \]_{(\nu)}-\bxi^\mu}\nonumber\\
&\le 
m+m\beta \norm{\sum^{\kappa}_{\nu=1} \(\[ \bm{\Xi}^\sT \bx \]_{(\nu)}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\beta\kappa}\)\frac{\bxi_{(\nu)}}{m}}
\annot{By \eqref{eqn:sparsemax_upper_identity}}\\
&= 
m+d^{\nicefrac{1}{2}}m\beta \[\sum^{\kappa}_{\nu=1}\( \[ \bm{\Xi}^\sT \bx \]_{(\nu)}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\beta\kappa}\)\]
\\
&\le 
m+d^{\nicefrac{1}{2}}m\beta \[\kappa \(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}\)+\frac{1}{\beta}\].
\end{align}
By the first inequality of \cref{coro:eps_sparse_dense}, for $\alpha\geq 2$, we have
\bea
\norm{\calT(\bx)-\bxi_\mu}\leq\norm{\calT_{\Sparsemax}(\bx)-\bxi_\mu}\leq m+d^{\nicefrac{1}{2}}m\beta \[\kappa \(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}\)+\frac{1}{\beta}\].
\eea
\end{proof}

\begin{remark}[Noise-Robustness]
    In cases of contaminated patterns with noise $\bm{\eta}$, i.e. $\Tilde{\bx}=\bx+\bm{\eta}$ (noise in query) or $\Tilde{\bxi}_\mu=\bxi_\mu+\bm{\eta}$ (noise in memory), the impact of noise $\bm{\eta}$ on the sparse retrieval error ($\alpha\geq2$) \eqref{eqn:eps_sparse_over_2} is linear, while its effect on the dense retrieval error ($2\geq\alpha\geq1$)\eqref{eqn:eps_sparse_dense} is exponential.
\end{remark}


\begin{theorem}
\label{thm:well_separation_condition}
Suppose $\delta\coloneqq \norm{\calT_{\text{Dense}}-\bxi_\mu}-\norm{\calT-\bxi_\mu}$.
Then, the {well-separation} condition can be formulated as:
\bea
\Delta_\mu \ge 
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR.
\eea
Furthermore, if $\delta=0$, this bound reduces to {well-separation} condition of Softmax-based Hopfield model.
\end{theorem}
\begin{proof}
Let $\calT_{\text{Dense}}$ be the retrieval dynamics given by the dense modern Hopfield model \cite{ramsauer2020hopfield},
and $\epsilon_{\alphaentmax}\coloneqq \norm{\calT(\bx)-\bxi_\mu}$ and $\epsilon_{\text{Dense}}\coloneqq\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}$ be the retrieval error of generalized and dense Hopfield model, respectively.

By \cref{coro:eps_sparse_dense}, we have
\bea
\label{eqn:eps_sparse_dense}
\epsilon_{\Sparsemax}=\norm{\calT(\bx)-\bxi_\mu} 
&\leq& \epsilon_{\text{Dense}}=
\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}.
\eea

Next we want to find the lower bound of separation $\Delta_\mu$ such that $\calT$ is a mapping from $S_\mu$ onto $ S_\mu$. 
To connect $\calT$ with $\Delta_\mu$, first we derive the bound on $\norm{\calT(\bx)-\bxi_\mu}$ via \cite[Lemma~A.4]{ramsauer2020hopfield}
\begin{align}
&\quad\quad\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}\\
&=
\norm{\bxi_\mu-\sum^M_{\nu=1} [\Softmax(\beta \Xi^\sT \bx)]_\nu \bxi_\nu}\\
&=
\norm{\(1-\[\Softmax(\beta \Xi^\sT \bx)\]_\mu\)\bxi_\mu-\sum^M_{\nu=1, \nu \neq \mu}\[\Softmax(\beta \Xi^\sT \bx)\]_\nu\bxi_\nu}\\
&\leq
\tilde{\epsilon} \norm{\bxi_\mu}+\frac{\tilde{\epsilon}}{M-1}\sum^M_{\nu=1, \nu \neq \mu} \norm{\bxi_\nu}\\
&\le 
\tilde{\epsilon} \( m+\frac{1}{M-1}\sum^M_{\nu=1, \nu \neq \mu} m\)
\\
\label{eqn:bound_eps}
&\leq
2\tilde{\epsilon} m,
\end{align}
where $\tilde{\epsilon}\coloneqq (M-1)\exp{-\beta \tilde{\Delta}_\mu}
=(M-1)\exp{-\beta \(\Braket{\bxi_\mu,\bx}-\Max_{\nu\in[M]}\Braket{\bxi_\mu,\bxi_\nu}\)}
$ and the upper bound on $\Softmax$
\bea
\[\Softmax(\beta \Xi^\sT \bx)\]_\nu
=\frac{\exp{\beta\(\Braket{\bx,\bxi_\nu}-\Braket{\bx,\bxi_\mu}\)}}{1+\sum_{\nu'\neq \mu} \exp{\beta\(\Braket{\bx,\bxi_{\nu'}}-\Braket{\bx,\bxi_\mu}\)}}
\le 
\exp{-\beta \Tilde{\Delta}_\mu},
\eea is inserted in the fourth line.
Then, by the Cauchy-Schwartz inequality
\bea
\abs{\Braket{\bxi_\mu,\bxi_\mu}-\Braket{\bx,\bxi_\mu}}
\leq
\norm{\bxi_\mu-\bx} \cdot \norm{\bxi_\mu}
\leq
\norm{\bxi_\mu-\bx}m,\quad\forall \mu\in [M],
\eea
we observe that $\tilde{\Delta}_\mu$ can be expressed in terms of $\Delta_\mu$: 
\begin{align}
\Tilde{\Delta}_\mu 
&=
\Min_{\nu,\nu\neq \mu}
\[
\Braket{\bx,\bxi_\mu}-\Braket{\bx,\bxi_\nu}
+
\(\Braket{\bxi_\mu,\bxi_\mu}-\Braket{\bxi_\mu,\bxi_\nu}\)
-
\(\Braket{\bxi_\mu,\bxi_\mu}-\Braket{\bxi_\mu,\bxi_\nu}\)
\]
\\
&
\geq \Min_{\nu,\nu\neq \mu}
\[
\Braket{\bxi_\mu,\bxi_\mu}-\Braket{\bxi_\mu,\bxi_\nu}
+
\(\Braket{\bxi_\mu,\bxi_\nu}-
\Braket{\bx,\bxi_\nu}\)
-
\(\Braket{\bxi_\mu,\bxi_\mu}-
\Braket{\bx,\bxi_\mu}\)
\]
\annot{By Cauchy-Schwarz}
\\
&=
\Delta_\mu - 2 \norm{\bxi_\mu-\bx}m=\Delta_\mu-2mR,
\annot{By $\bx\in  S_\mu$}
\end{align}
where $R$ is radius of the sphere $S_{\mu}$.
Thus, inserting the upper bound given by \eqref{eqn:bound_eps} into \eqref{eqn:eps_sparse_dense}, we obtain
\bea
\norm{\calT(\bx)-\bxi_\mu}
&\leq&
\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu} 
\leq 
2 \Tilde{\epsilon} m\\
&=&
2(M-1)\exp{-\beta \Tilde{\Delta}_\mu}m\\
&\leq&
2(M-1) \exp{-\beta\(\Delta_\mu-2mR\)}m.
\eea
Then, for any given $\delta\coloneqq \norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}-\norm{\calT(\bx)-\bxi_\mu}\le 0 $, the retrieval error $\norm{\calT(\bx)-\bxi_\mu}$ has an upper bound:
\bea
\norm{\calT(\bx)-\bxi_\mu} \le 2(M-1) \exp{-\beta\(\Delta_\mu-2mR +\delta\)}m - \delta
\le \norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu} .
\eea
Therefore, for $\calT$ to be a mapping $\calT:S_\mu\to S_\mu$, it is sufficient to obtain
\bea
2(M-1) \exp{-\beta(\Delta_\mu-2mR)}m  - \delta
\leq
R,
\eea
which implies that
\bea
\Delta_\mu
\geq
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR.
\eea
\end{proof}

\begin{lemma}[Memory Capacity Lower Bound]
\label{thm:memory_capacity}
Suppose the probability of successfully storing and retrieving memory pattern  is given by $1-p$.
The number of memory patterns sampled from a sphere of radius $m$ that the sparse Hopfield model can store and retrieve has a lower bound:
\bea
M \ge \sqrt{p}C^\frac{d-1}{4},
\eea
where $C$ is the solution for $C=\nicefrac{b}{W_0({\exp\{a+\ln{b}\}})}$ with $W_0(\cdot)$ being the principal branch of Lambert $W$ function \cite{olver2010nist}, $a\coloneqq \nicefrac{4}{d-1}\big\{\ln\[\nicefrac{2m(\sqrt{p}-1)}{(R+\delta)}\]+1\big\}$ and $b\coloneqq \nicefrac{4m^2\beta}{5(d-1)}$.
For sufficiently large $\beta$, the sparse Hopfield model has a larger lower bound on the exponential-in-d memory capacity compared to that of dense counterpart \cite{ramsauer2020hopfield}:
$
M\ge M_{\text{Dense}}.
$
\end{lemma}
\begin{proof}
To calculate the lower bound on the number of stored memory patterns, here we begin with an auxiliary lemma.
\begin{lemma}[\cite{ramsauer2020hopfield}]
\label{lemma:W} 
If the identity
\begin{equation}
ac + c\ln{c} - b = 0,
\end{equation}
holds for all real numbers $a, b \in \mathbb{R}$, then $c$ takes a solution:
\begin{equation}
c = \frac{b}{W_0(\exp(a+\ln{b}))}.
\end{equation}
\end{lemma}
\begin{proof}
With the given equation $ac + c\ln{c} - b = 0$, we solve for $c$ by following steps:
\begin{align*}
ac + c\ln{c} - b &= 0, \\
a + \ln{c} &= \frac{b}{c}, \\
\frac{b}{c} + \ln\left(\frac{b}{c}\right) &= a + \ln{b}, \\
\frac{b}{c}\exp\left(\frac{b}{c}\right) &= \exp(a + \ln{b}), \\
\frac{b}{c} &= W_0(\exp(a + \ln{b})), \\
c &= \frac{b}{W_0(\exp(a + \ln{b}))}.
\end{align*}
Q.E.D.
\end{proof}
Then we begin the main proof text.
Here we define $\Delta_{\min}$ and $\theta_{\mu\nu}$ as $\Delta_{\min}\coloneqq\Min_{\mu\in[M]}\Delta_\mu$ and the angle between two patterns $\bxi^\mu$ and $\bxi^\nu$, respectively. 
Intuitively, $\theta_{\mu\nu}\in[0,\pi]$ represent the pairwise correlation of two patterns the two patterns.

We have
\bea
\Delta_{\min}\ge 
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR,
\eea
and
\bea
\Delta_{\min}=\Min_{1\le\mu\le\nu\le M}\[m^2\(1-\cos{\theta_{\mu\nu}}\)\]
=m^2 \[1-\cos{\theta_{\min}}\],
\eea
where $\theta_{\min}\coloneqq \Min_{1\le\mu\le\nu\le M} \theta_{\mu\nu}\in[0,\pi]$.
Then, the last inequality can be rewritten as
\bea
\label{eqn:cos}
m^2 \[1-\cos{\theta_{\min}}\] 
\ge 
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR.
\eea

Following the well separation condition 
$\Delta_\mu \ge 
    \frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR
    $ given by \cref{thm:well_separation_condition}, here we formulate the probability of successful storage and retrieval, i.e. minimal separation $\Delta_{\min}$ satisfies \cref{thm:well_separation_condition}.
\bea
P\(\Delta_\mu\ge \frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR \)= 1-p.
\eea
Inserting \eqref{eqn:cos} into last inequality, we obtain:
\bea
\label{success}
P\( m^2 \[1-\cos{\theta_{\min}}\] \ge  \frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR \) = 1-p.
\eea
From \cite[(4.22.2)]{olver2010nist}, for $0 \le \cos{\theta_{\min}} \le 1$, $\cos{\theta_{\min}}$ has an upper bound:
\bea
\cos{\theta_{\min}} \le 1- \frac{\theta_{\min}^2}{5}.
\eea
It holds
\bea
P\( \frac{m^2\theta_{\min}^2}{5} \ge \frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR\)= 1-p,
\eea
which can be reformulated as
\bea
P\(M^{\frac{2}{d-1}}\theta_{\min} \ge \frac{\sqrt{5}M^{\frac{2}{d-1}}}{m}\[\frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR\]^\half\) = 1-p.
\label{eqn:ineq1}
\eea
For later convenience, here we introduce $M^{\nicefrac{2}{d-1}}$.

Here we define
\bea
\omega_d
\coloneqq 
\frac{2\pi^{\nicefrac{d+1}{2}}}{\Gamma\(\frac{d+1}{2}\)},
\eea
as the manifold area of a $d$-dimensional unit sphere, where $\Gamma(\cdot)$ represents the gamma function.



Following \cite[Lemma~3.5]{brauchart2018random}, we have
\begin{align}
P&\(M^{\frac{2}{d-1}}\theta_{\min} \ge \frac{\sqrt{5}M^{\frac{2}{d-1}}}{m}\[\frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR\]^{\half}\)
= 1-p
\nonumber\\
&\quad\quad\quad\ge
1-\half\gamma_{d-1}5^{\frac{d-1}{2}}M^2 m^{-(d-1)}\[\frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR\]^{\frac{d-1}{2}},
\label{eqn:ineq2}
\end{align}
where $\gamma_d$ is characterized as the quotient between the surface areas of the unit spheres in $(d-1)$ and $d$ dimensions, respectively:
\bea
\gamma_d \coloneqq \frac{1}{d} \frac{\omega_{d-1}}{\omega_d}=\frac{1}{d\sqrt{\pi}}\frac{\Gamma\(\frac{d+1}{2}\)}{\Gamma\(\frac{d}{2}\)}.
\eea
Recall $d, M\in \mathbb{N}_+$, $p\in [0,1]$. 
The equation
\bea
M=\sqrt{p}C^{\frac{d-1}{4}}
\eea
holds for some real values $C\in\R$.
By \eqref{eqn:ineq2}, we obtain
\bea
5^{\frac{d-1}{2}}
    \(\sqrt{p}C^{\frac{d-1}{4}}\)^2 m^{-(d-1)}\Bigg\{\frac{1}{\beta}\ln{\[\frac{2\(\sqrt{p}C^{\frac{d-1}{4}}-1\)m}{R+\delta}\]}+\frac{1}{\beta}\Bigg\}^{\frac{d-1}{2}}-p \le 0,
\eea
and thus
\bea
5^{\frac{d-1}{2}}C^{\frac{d-1}{2}} m^{-(d-1)}\Bigg\{\frac{1}{\beta}\ln{\[\frac{2\(\sqrt{p}C^{\frac{d-1}{4}}-1\)m}{R+\delta}\]}+\frac{1}{\beta}\Bigg\}^{\frac{d-1}{2}}\le 1.
\label{eqn:ineq3}
\eea

To apply \cref{lemma:W}, here we reformulate \eqref{eqn:ineq3} as
\bea
\frac{5C}{m^2\beta}\Bigg\{\ln\[\frac{2\(\sqrt{p}C^{\frac{d-1}{4}}-1\)m}{R+\delta}\]+1\Bigg\}-1 \leq 0,
\eea
and define
\bea
\label{eqn:identified_ab}
a\coloneqq \frac{4}{d-1}\Bigg\{\ln\[\frac{2m(\sqrt{p}-1)}{R+\delta}\]+1\Bigg\}, 
\quad 
b\coloneqq \frac{4m^2\beta}{5(d-1)}.
\eea

By \cref{lemma:W}, $C$ can be expressed as
\bea
\label{eqn:c}
C=\frac{b}{W_0({\exp\{a+\ln{b}\}})},
\eea
where $W_0(\cdot)$  is the upper branch of the Lambert $W$ function.
Since the domain of the Lambert $W$ function is $x>(-\nicefrac{1}{e},\infty)$ and {the fact $\exp{a+\ln{b}}>0$}, the solution for \eqref{eqn:c} exists.

When the inequality \eqref{eqn:ineq3} holds, the lower bound on the exponential storage capacity $M$ can be written as:
\bea
M
\geq
\sqrt{p}C^{\frac{d-1}{4}}.
\eea
In particular, the above lower bound takes a form similar to \cite[Theorem~3]{ramsauer2020hopfield}.
To observe the advantages induced by sparsity, we conduct the following asymptotic analysis and compare it with results from the dense counterparts.
To compare with results from dense modern Hopfield model, we denote the dense counterparts of  $a,b$ with $\Tilde{\cdot}$ notation, i.e. 
\bea
\Tilde{a}\coloneqq \frac{2}{d-1} \[1+\ln{\(2\beta m^2 p\)}\],\quad \Tilde{b}=b.
\eea

By \cite{corless1996lambert}, for sufficient large $z$, $W_0(z)$ can be approximated as
\bea
W_0(z)\simeq \ln{z} - \ln{\ln{z}}+\calO(1).
\eea

Therefore,
with sufficient large $\beta$, we have
\bea
W_0\(\exp{a+\ln b}\)\simeq
a+\ln b-\ln\({a+\ln b}\)+\calO(1),
\eea
where $a$ is the predominance.

For $a$, the inequality
\bea
\Tilde{a}\leq a
\eea
holds, which leads to
\bea
W_0\(\exp{\Tilde{a}+\ln \Tilde{b}}\)
\leq
W_0\(\exp{a+\ln b}\).
\eea
Therefore, combining the last inequality with \eqref{eqn:c}, we obtain
\bea
\Tilde{C} = \frac{b}{W_0\(\exp{\Tilde{a}+\ln \Tilde{b}}\)} \leq \frac{b}{W_0\(\exp\{a+\ln b\}\)} = C,
\eea
which implies that the capacity lower bound of sparse Hopfield models is greater than that of \cite{ramsauer2020hopfield}
\bea
M=\sqrt{p}C^{\frac{d-1}{4}}
\geq
\sqrt{p}\Tilde{C}^{\frac{d-1}{4}}=M_{\text{Dense}}.
\eea
\end{proof}

==> boarder.tex <==
To be filled.
